Paint by Inpaint: Learning to Add Image Objects by Removing Them First

Image editing has advanced significantly with the introduction of text-conditioned diffusion models. Despite this progress, seamlessly adding objects to images based on textual instructions without requiring user-provided input masks remains a challenge. We address this by leveraging the insight that removing objects (Inpaint) is significantly simpler than its inverse process of adding them (Paint), attributed to inpainting models that benefit from segmentation mask guidance. Capitalizing on this realization, by implementing an automated and extensive pipeline, we curate a filtered large-scale image dataset containing pairs of images and their corresponding object-removed versions. Using these pairs, we train a diffusion model to inverse the inpainting process, effectively adding objects into images. Unlike other editing datasets, ours features natural target images instead of synthetic ones while ensuring source-target consistency by construction. Additionally, we utilize a large Vision-Language Model to provide detailed descriptions of the removed objects and a Large Language Model to convert these descriptions into diverse, natural-language instructions. Our quantitative and qualitative results show that the trained model surpasses existing models in both object addition and general editing tasks. Visit our project page for the released dataset and trained models at https://rotsteinnoam.github.io/Paint-by-Inpaint.

==> filtering_table.tex <==
\begin{table}[t]
\setlength\tabcolsep{0pt}
\caption{
\textbf{Datasets Comparison.}
Review of \pipe{} with other editing datasets.
\ding{51} signifies fulfillment,
\ding{55} indicates non-fulfillment,
and {\ding{51}\raisebox{-0.9ex}{\textsuperscript{\kern-0.9em\scalebox{1.6}{\ding{55}}}}} denotes partial fulfillment,
where images are real outside inpainted areas.
"\textbf{--}" means no such images available.
"General Classes" indicates dataset class diversity.
}
\vspace{-0.15cm}
\begin{tabular*}{1.03\linewidth}{@{\extracolsep{\fill}}lcccccc} 
\toprule

{\textbf{Dataset}} & { Initial} & {Passed} & {Passed} & {Passed} & {{Passed}}\\
\vspace{-13pt} \\
{} & {Annotations} & {Pre-} & {Consensus}  & {Multimodal} & {Importance}\\
{} & {} & {Removal} & {CLIP}  & {CLIP} & {Filtering}\\

\midrule
COCO & 591K & 329K & 234K & 205K & 187K\\
LVIS  & 1270K & 314K& 235K& 212K& 191K\\
OpenImages  & 2,785K & 851K& 632K&569K &510K\\
\bottomrule 
\end{tabular*}
\label{Table:datasets}
\vspace{-0.4cm}
\end{table}


==> sec/limitations.tex <==
\vspace{-0.23cm}
\section{Limitations}
\vspace{-0.25cm}
\label{sec:limitations}

Despite the impressive results produced by our model, several limitations remain. First, while our data curation pipeline improves robustness during the removal phase, it is not entirely error-free. Additionally, the model struggles with significant changes occurring far from the object but are affected by it. For instance, it handles nearby effects, like TV shadows (see \cref{Fig:Visual_Result_Teaser} and \cref{SM_figure:limitations}), but struggles with larger shadows or distant reflections, as seen in the center images of \cref{SM_figure:limitations}. Similarly, object-object interactions are not always accurately handled (see the right images in the figure). These challenges stem from the dataset construction, as our method minimizes alterations outside the near-object region. Future work could explore inpainting both the object and distant regions influenced by it. We hope our work inspires future research to address these limitations.

